Semi-supervised Learning of Pushforwards For Domain Translation & Adaptation

Given two probability densities on related data spaces, we seek a map pushing one density to the other while satisfying application-dependent constraints. For maps to have utility in a broad application space (including domain translation, domain adaptation, and generative modeling), the map must be available to apply on out-of-sample data points and should correspond to a probabilistic model over the two spaces. Unfortunately, existing approaches, which are primarily based on optimal transport, do not address these needs. In this paper, we introduce a novel pushforward map learning algorithm that utilizes normalizing flows to parameterize the map. We first re-formulate the classical optimal transport problem to be map-focused and propose a learning algorithm to select from all possible maps under the constraint that the map minimizes a probability distance and application-specific regularizers; thus, our method can be seen as solving a modified optimal transport problem. Once the map is learned, it can be used to map samples from a source domain to a target domain. In addition, because the map is parameterized as a composition of normalizing flows, it models the empirical distributions over the two data spaces and allows both sampling and likelihood evaluation for both data sets. We compare our method (parOT) to related optimal transport approaches in the context of domain adaptation and domain translation on benchmark data sets. Finally, to illustrate the impact of our work on applied problems, we apply parOT to a real scientific application: spectral calibration for high-dimensional measurements from two vastly different environments

==> mnist.tex <==
% Text about digits/USPS/MNIST took out of main
 before evaluating our method for domain adaptation on the USPS and MNIST digits datasets
 
 Then, we apply our method to learn a mapping that improves prediction on the USPS digits dataset using a model trained on MNIST digits (Setion~\ref{sec:digits}). 
 
 domain adaptation on the USPS and MNIST digits datasets (Section~\ref{sec:digits}), 
 
 For the USPS and MNIST datasets, we show that the learned transformation improves classification of USPS digits with models trained on MNIST digits.
 
 \subsection{USPS and MNIST} \label{sec:digits}
We load the USPS and MNIST data sets from \texttt{torchvision} and standardize by mean 0.5, scale 0.5. We center crop the 32 $\times$ 32 MNIST images to 24 $\times$ 24 then resize to 16 $\times$ 16 to match the size of the USPS digits. We split the training set into 80\% training data and 20\% validation data and use the test sets as is. We generate paired data as follows. For each class label, we select $N_p = 20$ pairs by first randomly selecting a USPS digit image, then selecting the closest (in Euclidean distance) MNIST digit image. To evaluate domain adaptation, we train two classification models: Model 1, a modified LeNet5 mapping from 16 $\times$ 16 greyscale images to classification scores, and Model 2, a classifier mapping from a latent representation dimension ($d = 30$) to classification scores. 
Model 1 is trained on the MNIST training set; we find that it performs well on the MNIST test set but not the USPS test set (Table \ref{tab:digits_results}).
Model 2 is trained on the parOT latent representations corresponding to translated MNIST-to-USPS data; that is, we learn the parOT map between the two domains, then map MNIST to the USPS latent representation, then train a new classifier.
This model performs better on USPS data than Model 1.

\begin{table}[]
    \centering
    \caption{Caption}
    \label{tab:digits_results}
    \begin{tabular}{l|l|r|r}
        Model & Training data & Test acc. & USPS test acc. \\ \hline
        Model 1 & MNIST & 97.6 & 77.2 \\
        Model 2 & MNIST-to-USPS & 97.8 & 86.0
    \end{tabular}
\end{table}

The implementation details for parOT applied to MNIST and USPS are as follows. As an encoder to latent dimension 30, we use the LeNet trained on MNIST images but remove the final classification layer. We leave this encoder fixed while learning a convolutional decoder trained on both the USPS and MNIST images. Examples of digits and their reconstructions via this autoencoder are shown in Figure~\ref{fig:digits_ae}. Once the autoencoder is learned in an unsupervised fashion, we leave it fixed during fitting of parOT. We leave design of better autoencoders to future work and note that our domain adaptation is performed in the latent space to avoid issues with reconstruction artifacts.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{ArXiv/Figs/parOTDigitsAE.png}
    \caption{Caption}
    \label{fig:digits_ae}
\end{figure}

For the parOT model, we use a combination of an affine transformation and 64 RealNVP coupling layers on the 30-dimensional latent space. After training, we inspect the quality of translation from MNIST to USPS; Figure~\ref{fig:digits_trans} shows randomly chosen example digits translated from MNIST to USPS. Here, it is difficult to disentangle potential inaccuracies of the autoencoder from the domain translation mapping, but we do note that in many cases, the translation is capturing the digit shape while making the translated digit a bit blurrier (which qualitatively matches the USPS dataset).

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{ArXiv/Figs/parOTDigitsTrans.png}
    \caption{Caption}
    \label{fig:digits_trans}
\end{figure}
